SMH-Bench: Benchmarking LLM Agents for Environment-Grounded Reasoning and Action in Smart Homes

Smart homes are evolving toward complex state-dependent living environments, requiring Large Language Models (LLMs) to reason over user intent, preferences, and multi-device interactions. However, existing smart-home benchmarks often focus on static instruction-to-API mapping or limited simulations, failing to evaluate whether LLMs can reason, interact, and act reliably in realistic household scenarios. To address these limitations, we introduce SMH-Bench, a comprehensive benchmark for evaluating LLMs in smart-home environments. Built upon HomeEnv, an executable and verifiable smart-home simulator, SMH-Bench contains 1,100 high-quality tasks spanning 7 categories and 22 fine-grained subcategories. It further stratifies tasks across simple, medium and complex homes, ranging from small apartments to dense multi-room environments with 135 devices. Experiments show that although frontier LLMs achieve strong performance on explicit control and query tasks, they still exhibit significant weaknesses in automation task scheduling, ambiguity handling and personalized reasoning, especially as home complexity increases. We hope SMH-Bench will facilitate the development of more reliable, context-aware, and practically deployable smart-home agents.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: The abstract and Introduction state the paper's main contribution as SkillGenBench, a benchmark for evaluating skill-generation pipelines. They also describe the benchmark scope, including task-conditioned and task-agnostic generation, repository- and document-grounded sources, fixed downstream execution, and the reported empirical study.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: Appendix~\ref{sec:limitations} includes a Limitations section that discusses the current dynamic coverage of generation backbones, the diagnostic nature of the failure taxonomy, the focus on deterministic verifiers and fixed downstream execution, the non-exhaustive source coverage, and the limitations of static rule-based scores.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper introduces a benchmark and empirical evaluation protocol, and does not present theoretical results, theorems, or formal proofs.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    \item[] Justification: Section~\ref{sec:exp_setup} specifies the evaluated methods, generation backbones, fixed downstream executor, pass@3 metric, verifier-based success criterion, three-trial evaluation setting, and 1800-second per-instance budget. Appendix~\ref{app:baselines} and Appendix~\ref{app:runtime_details} provide baseline adaptations, runtime controls, Docker-based execution setting, API settings, token limits, and time limits needed to reproduce the reported results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}
    \item[] Justification: We provide an anonymized dataset release at \url{https://huggingface.co/datasets/anonymous-skillgenbench/SkillGenBench} and an anonymized code release at \url{https://anonymous.4open.science/r/SkillGenBench-3EE3/}. These releases include benchmark materials, evaluation bundles, baseline/evaluation code, and reproduction instructions for the reported SkillGenBench runs.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: Section~\ref{sec:exp_setup} describes the evaluated skill-generation methods, six generation backbones, fixed MiniMax-2.5 downstream executor, verifier-based success criterion, pass@3 metric, three-trial setting, and 1800-second per-instance evaluation budget. Appendix~\ref{app:baselines} and Appendix~\ref{app:runtime_details} provide baseline adaptation details, Docker-based environment settings, API/runtime controls, token-budget handling, and time limits. No training optimizer or data split is involved because the paper evaluates skill-generation pipelines rather than training new models.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: Appendix~\ref{app:bootstrap_ci} reports task-level bootstrap 95\% confidence intervals for the overall pass@3 results in Table~\ref{tab:main_results}. The paper draws $B{=}2000$ bootstrap resamples with replacement over the 187 benchmark tasks, computes pass@3 on each resample, and reports the mean and confidence-interval bounds in Table~\ref{tab:bootstrap_ci}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: The experiments do not train or fine-tune models locally; skill generation and downstream execution are performed through hosted model APIs, so provider-side CPU/GPU worker type, memory, and storage are not exposed to or controlled by the authors. Appendix~\ref{app:runtime_details} reports the reproducibility-relevant compute configuration: the shared SkillGenBench harness, Claude Code CLI and SDK versions, six hosted generation backbones, fixed MiniMax-2.5 downstream executor, Docker-based isolated downstream execution, no local GPU usage, temperature, max output tokens, and 1800-second timeouts. Section~\ref{sec:exp_setup} further reports the pass@3 setting with up to three independent trials per instance over the 187-task benchmark.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}
    \item[] Justification: The work is a benchmark and empirical evaluation study using released benchmark materials, documented source boundaries, and controlled execution environments. We are not aware of any aspect of the research process that violates the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}
    \item[] Justification: Appendix~\ref{sec:limitations} includes a Broader Impact paragraph discussing the potential benefit of improving reliable evaluation for agent systems, as well as risks from misuse of generated workflows and reduced barriers to executing complex tasks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper releases a benchmark dataset and evaluation code, not a pretrained model, image generator, or other high-risk generative model. The release is intended for controlled benchmark evaluation and does not introduce a separately deployable generative system requiring model-release safeguards.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification: Existing assets used in the benchmark and baseline implementations are credited through the paper citations and release documentation, and the anonymized release includes license information for the benchmark package and source materials. We include only assets whose terms permit research redistribution or evaluation use.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{}
    \item[] Justification: SkillGenBench is released as a new benchmark asset with an anonymized dataset release at \url{https://anonymous.4open.science/r/SkillGenBench-3EE3/} and an anonymized code release at \url{https://anonymous.4open.science/r/SkillGenBench-3EE3/}. The release includes benchmark materials, task manifests, evaluation bundles, code, and dataset documentation, including a dataset card and Croissant metadata. Consent for human-subject data is not applicable because the benchmark does not collect participant data or involve a human-subjects study.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper does not involve crowdsourcing experiments or research with human subjects. The manual verification described in Appendix~\ref{app:human_verification} was an internal benchmark-construction audit rather than a human-subjects study.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification: No study participants are recruited and no participant data, interventions, surveys, or behavioral measurements are collected in this work. The internal benchmark-item audit does not constitute human-subjects research, so IRB approval or equivalent review is not applicable.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerYes{}
    \item[] Justification: LLMs are central to both benchmark construction and evaluation. Section~\ref{sec:exp_setup} describes the LLM backbones used for skill generation and the fixed MiniMax-2.5 downstream executor used for evaluation. Appendix~\ref{app:runtime_details} documents the generation API setting, Claude Code runtime, and evaluation API settings, and Appendix~\ref{app:prompts:gen} lists the prompts used for knowledge-graph construction, scenario generation, task/test-case generation, validation, and refinement.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> sections/3.benchmark_backup.tex <==
\section{SMH-Bench}



% To evaluate smart-home agents under realistic household interactions, we construct \textbf{SMH-Bench}, a closed-loop benchmark for executable smart-home tasks. Unlike evaluations that reduce user instructions to isolated device API calls, SMH-Bench models a home as an executable world composed of rooms, devices, attributes, services, and environment states. Each task contains not only a natural-language request, but also an initial home state, available device capabilities, reference state changes, and executable verification conditions. An agent must understand the user intent in the given home, ground references to devices, select services, infer arguments, handle ambiguity or context, and eventually drive the home state to the desired outcome.

% SMH-Bench follows four design principles. First, tasks should reflect real smart-home interactions rather than isolated function calls: user requests may be colloquial, noisy, underspecified, multi-turn, or dependent on the current device state. Second, environments must be reproducible: each home state is described by a structured engine and can be reconstructed by the simulator. Third, evaluation should be based on final states rather than exact action-sequence matching, since multiple valid action paths may lead to the same outcome. Fourth, the benchmark should cover the full assistant loop, including direct execution, state query, automation-rule generation, clarification, multi-turn reference resolution, and memory constraints.

\subsection{Task Formulation}

% Each SMH-Bench instance is represented as a tuple
% \[
% x=(q,E,H,G,c),
% \]
% where $q$ is the user instruction, $E$ is the initial home environment, $H$ is optional dialogue history, $G$ is the reference output, including state-change labels, automation conditions, or query responses, and $c$ is an executable critic expression for final-state verification. The environment $E$ contains rooms, devices, device attributes, service definitions, service argument constraints, and current states. Given $q$, $E$, and $H$, a model must produce actions, automation rules, clarification questions, or natural-language answers.

% For control tasks, model actions are executed in the simulator. The evaluator compares pre- and post-execution state snapshots and normalizes model behavior into state-change labels:
% \[
% \Delta=\{(d_i,a_i,v_i)\},
% \]
% where $d_i$ is the device ID, $a_i$ is the attribute path, and $v_i$ is the resulting attribute value. The evaluator then executes the critic expression $c$ on the candidate final state to determine whether the home satisfies the target condition. Query tasks do not modify the environment and instead require factual answers about the current home state. Automation tasks require both trigger conditions and triggered device actions.

\subsection{Task Taxonomy}

SMH-Bench contains 1,100 benchmark instances spanning 7 major categories and 22 subcategories. The taxonomy is organized by the core capabilities required in realistic smart-home assistance, rather than by device type. Each subcategory is further divided into \textit{simple}, \textit{medium}, and \textit{complex} difficulty levels according to the complexity of the home state and required reasoning.

\paragraph{Atom.}
Atom tasks evaluate basic but necessary grounding ability. The \texttt{clear} subset contains instructions with explicit devices, rooms, and target values. The \texttt{colloquial} subset rewrites the same control goals into natural spoken expressions, such as ``close the curtains.'' The \texttt{noisy} subset introduces repetition, self-correction, or redundant phrases, requiring the model to recover the true operational intent from irregular input. These tasks usually involve one target device, but still require correct service selection and argument grounding.

\paragraph{Composite.}
Composite tasks emphasize the compositional nature of real household requests. \texttt{multi\_device} requires coordinated control of multiple devices or attributes. \texttt{batch\_control} requires selecting a set of devices by category or scope. \texttt{state\_dependent} requires reading current states before deciding the target set. \texttt{room\_dependent} requires filtering by room relations, occupancy signals, room type, or environmental sensors. \texttt{top\_n} requires ranking candidate devices or rooms, such as selecting the targets with the highest fan speed, humidity, or volume. These tasks extend single API calls into multi-step environment grounding and planning.

\paragraph{Ambiguous.}
Ambiguous tasks test whether a model knows when to infer and when to ask for clarification. \texttt{intent\_state} contains implicit state-oriented requests such as ``it feels stuffy here'' or ``the room is too dark,'' where the model must infer a reasonable action from the environment and available devices. \texttt{intent\_scene} contains scene-like expressions such as ``good morning'' or ``I want to relax,'' which usually need to be mapped to lighting, curtains, air conditioning, or media devices. \texttt{slot\_missing} deliberately omits key slots such as target room, device, mode, or duration. These samples include clarification turns in the history and evaluate whether the model asks necessary questions before execution.

\paragraph{Automation.}
Automation tasks require creating trigger-action rules rather than immediate execution. The \texttt{time} subset covers fixed or periodic time triggers. The \texttt{state} subset covers device- or sensor-state triggers. The \texttt{state\_time} subset requires both time and state conditions, such as ``if the kitchen temperature is still above 35 degrees at 2 p.m. every day.'' Each automation condition is normalized into \texttt{\{time\_cron, state\_expr\}}, while action effects are still verified through final-state labels and critic expressions. This design evaluates both trigger semantics and triggered device control.

\paragraph{Multiturn.}
Multiturn tasks simulate context dependence in household dialogue. \texttt{continuity} requires inheriting devices or arguments from previous turns. \texttt{shift} requires recognizing that the user has switched to a new device or room. \texttt{resolution} evaluates reference resolution across devices, rooms, or different devices in the same room. \texttt{correction} evaluates whether the model updates its plan when the user revises, cancels, or overrides previous parameters. These samples provide historical context through \texttt{initial\_chat\_history}; scoring verifies whether the current-turn target state is satisfied.

\paragraph{Memory.}
Memory tasks distinguish short-term and long-term information. \texttt{shortterm} depends on context established in recent dialogue turns and tests long-context robustness, for example ``set the bedroom curtains the same way'' or ``raise the temperature a bit more.'' \texttt{longterm} injects user preferences, device aliases, default rules, and constraints through \texttt{memory\_list}; for example, the user may call a device ``Xiao Hai,'' or the phrase ``I am going to sleep'' may correspond to a default routine. Memory is not evaluated by asking the model to restate memory text, but by whether the final actions satisfy the relevant preferences and constraints.

\paragraph{Query.}
Query tasks do not change the home state. They evaluate factual reading and expression over the environment. The \texttt{status} subset asks about device attributes or operating states, such as whether a vacuum is currently cleaning. The \texttt{quantity} subset asks for counts of devices satisfying certain conditions, such as the number of fans currently on. Since correctness is expressed in natural language rather than state changes, query tasks use a query-response judge to compare the core facts in model and reference answers.

The three difficulty levels provide horizontal comparability. \textit{Simple} retains the core challenge of a capability type. \textit{Medium} introduces more complex room, device, or state combinations. \textit{Complex} further increases environmental distractors, candidate devices, expression length, or cross-state reasoning. By maintaining a fixed simple/medium/complex ratio within each subcategory, SMH-Bench supports reporting overall performance, capability-specific performance, and difficulty sensitivity.

\subsection{Executable Smart-Home Environment}

\paragraph{Home-state modeling.}
SMH-Bench builds its executable smart-home environment on HomeEnv, or Midea Home Assistant. The core design of HomeEnv is configuration-as-logic: device capabilities are not implemented by hand-written classes for each category, but described through serializable configurations of generic elements such as \texttt{Attribute}, \texttt{Service}, \texttt{Domain}, \texttt{Component}, and \texttt{Entity}. A home is represented as an executable object tree: the root is \texttt{Home}, which contains \texttt{Room} and \texttt{Device} objects; each \texttt{Device} contains \texttt{Attribute} and \texttt{Service} objects; each \texttt{Service} specifies arguments, type constraints, value ranges, and executable code.

Device capabilities are defined by YAML schemas and compiled into executable objects at load time. The current HomeEnv configuration covers common smart-home domains including \texttt{light}, \texttt{climate}, \texttt{cover}, \texttt{media}, \texttt{fan}, \texttt{vacuum}, \texttt{lock}, \texttt{sensor}, \texttt{battery}, and \texttt{device}, with 34 concrete device templates. Since all devices follow the same syntax objects and serialization protocol, SMH-Bench maintains consistent execution semantics across different home layouts, device combinations, and state initializations.

\paragraph{Agent-environment interface.}
HomeEnv wraps \texttt{HomeEngine} as a Gymnasium-style \texttt{HomeEnv}, providing a unified agent-environment loop. An agent sends structured actions to \texttt{HomeEnv.step(action)}, and the environment returns \texttt{observation}, \texttt{reward}, \texttt{terminated}, \texttt{truncated}, and \texttt{info}. This interface allows different agent protocols to share the same environment entry point, while state transitions, error feedback, and termination signals are recorded consistently.

The action space contains five core operations. \texttt{control\_device} controls device services or directly modifies attributes. \texttt{query\_device} retrieves devices. \texttt{query\_room} returns room structure. \texttt{pyexec} and \texttt{pyeval} allow models to execute or evaluate code through a Pythonic interface. For tool-using agents, query actions provide environment retrieval. For code-based agents, PyVM allows models to programmatically filter, rank, count, and batch-control devices.

When a model produces a control action, the environment first locates the device by \texttt{did}, then locates the target service or attribute by \texttt{locator}. It checks argument names, types, and ranges before executing the service code and mutating the corresponding attribute values. For example, if the user asks to set the smart screen in the game room to 20\% volume, the model must locate the smart screen and call \texttt{set\_volume\_level(volume\_level=20)}. HomeEnv checks that \texttt{volume\_level} is a valid integer within the allowed range, and then updates the device's \texttt{volume\_level} from its initial value to 20.

\paragraph{Stateful and executable evaluation.}
This environment design turns smart-home tasks from static text-to-API-name mapping into state transitions in a constrained world. Model actions truly mutate the in-memory home object tree; query actions return current device capabilities and states; code execution produces traceable side effects on the same object graph; and final evaluation is grounded in the executed state rather than in the model's stated intent.

HomeEnv provides three guarantees for SMH-Bench. First, reproducibility: each sample environment can be reconstructed from a serialized engine. Second, constraint enforcement: service definitions, argument ranges, attribute types, and cron conditions are checked by schema. Third, diagnosability: wrong devices, wrong services, invalid arguments, code exceptions, unintended device modifications, and rule-blocked operations can all be recorded. This executable environment allows SMH-Bench to test whether an agent truly understands home state, device capability, and user goal, rather than merely generating plausible action text.

\subsection{Benchmark Construction}

SMH-Bench follows a goal-first construction principle. We do not first generate arbitrary natural-language instructions and then infer their labels afterward. Instead, each sample starts from a verifiable goal in an executable home environment, and only then synthesizes the corresponding user expression. This ensures that every instance has a clear initial state, executable action, target state, and evaluation basis. The construction pipeline has four stages: home-environment construction, verifiable goal sampling, natural-language and dialogue synthesis, and simulation-based validation with filtering.

\paragraph{Diverse initial homes.}
We first construct diverse initial home environments from two sources: automatically synthesized homes based on device schemas and room configurations, and homes converted from real or semi-real online household data. Each environment contains multiple rooms and devices. Each device has a unique ID, room assignment, category, subcategory, tags, initial attribute values, and callable services. To improve realism, the construction process introduces controlled variation, including different device states, composite device components, offline or unavailable devices, and cases requiring localization by room, device name, category, or tag.

\paragraph{Goal and action sampling.}
After obtaining an initial environment, the generator samples executable goals from device capabilities. For control tasks, it enumerates services of available devices and samples required arguments as well as some optional arguments from service definitions. For composite tasks, it samples multiple devices or services to form multi-action goals. For delay and automation tasks, it inserts time conditions or delayed operations into action sequences, making the samples closer to real user control habits.

Different task categories use different goal-sampling strategies. Atom tasks directly sample single-device single-service goals. Composite tasks add filtering, batch control, state dependence, or ranking constraints over device sets. Ambiguous tasks first construct a reasonable final goal and then intentionally weaken device, room, mode, or argument information in the user expression. Automation tasks jointly sample trigger conditions and triggered actions; time conditions, state conditions, and time-state conjunctions are normalized into evaluable structures in the final data. Multi-turn and Memory tasks first construct historical context, then make the current request depend on previous devices, previous arguments, user corrections, device aliases, or long-term preferences. Device Query tasks do not sample state-changing actions, but instead extract answerable device facts or quantity-counting targets from the current environment.

\paragraph{Natural-language and dialogue synthesis.}
Once the goal is fixed, we use templates and LLMs to generate user requests. Templates ensure that target devices, services, and arguments are accurately covered, while LLMs produce more natural colloquial, noisy, ambiguous, and multi-turn expressions. For samples requiring clarification, the user request intentionally omits key slots, and a user simulator generates the subsequent user reply. For multi-turn samples, the generator continues producing follow-up queries to create continuity, topic shift, reference resolution, and correction. Each sample stores both dialogue and \texttt{system\_info}, so that later inference and evaluation can reconstruct the full home context observed by the model.

\paragraph{Simulation validation and human review.}
Finally, we filter candidate samples using the simulator and evaluator. Each candidate must satisfy three requirements: the reference actions must execute successfully in HomeEnv; the resulting state changes must match the ground-truth labels; and the critic expression must evaluate to true on the final state. For query tasks, we check that the reference answer is supported by the current environment state. For clarification tasks, we keep samples that require missing slots or unresolved intent to be clarified before safe execution. After automatic validation and human review, we obtain 1,100 benchmark instances.

\subsection{Evaluation Protocol}

SMH-Bench adopts simulator-grounded evaluation for executable and reproducible closed-loop assessment. The objective is not to check whether a model reproduces a labeled action sequence, but whether its behavior in the given home environment leads to the correct final home state without unintended side effects. The evaluator first runs model inference and records model outputs, tool calls, or code execution traces. It then normalizes behavior under different interaction protocols into a prediction record, a final engine snapshot, and token usage. Finally, the evaluation pipeline performs task-specific state verification, automation-condition verification, query-answer verification, and clarification verification, and aggregates the final result.

\paragraph{State-based control evaluation.}
For device-control tasks, the evaluator executes model actions in HomeEnv and computes the state difference before and after execution. The predicted state changes are then applied to a copy of the initial environment, and the critic expression is executed on the candidate final state. A model passes only if the target state satisfies the critic and devices not referenced by the critic remain unchanged. This design accepts different valid action paths that lead to the same correct final state, while penalizing over-execution and side effects.

\paragraph{Automation evaluation.}
For automation tasks, evaluation covers both action effects and trigger conditions. Time conditions are compared by sampling future trigger sequences from a fixed time anchor. State conditions are parsed as expressions and compared through symbolic equivalence or structured rules.

\paragraph{Query and clarification evaluation.}
For query tasks, the evaluator compares the core facts in the model answer and the reference answer using an LLM judge, including device states, counts, numeric values, room assignments, and attribute values. For clarification tasks, the model must ask a clarification question at the required turn. Under the strict setting, the judge further checks whether the question targets the missing information needed to resolve the intent.

\paragraph{Interaction protocols.}
SMH-Bench supports three agent interaction protocols. The context-only protocol provides the full home JSON to the model and requires a one-shot structured output containing actions or automation rules. The tool-augmented protocol exposes \texttt{query\_device}, \texttt{query\_room}, and \texttt{control\_device}, allowing the model to iteratively inspect the environment and act. The code-based protocol allows the model to access home objects through a Python interface, which is useful for complex filtering, ranking, and batch control. All three protocols are normalized into the same prediction schema and can therefore be compared under the same evaluation metrics.

Overall, SMH-Bench advances smart-home agent evaluation from static text matching to executable, reproducible, and diagnosable state verification. It evaluates not only whether a model can call the correct device API, but also whether it can complete realistic household assistant tasks under multi-room, multi-device, multi-turn, contextual, and preference-constrained settings.

